Fusing Neural and Physical: Augment Protein Conformation Sampling with Tractable Simulations

The protein dynamics are common and important for their biological functions and properties, the study of which usually involves time-consuming molecular dynamics (MD) simulations in silico. Recently, generative models has been leveraged as a surrogate sampler to obtain conformation ensembles with orders of magnitude faster and without requiring any simulation data (a "zero-shot" inference). However, being agnostic of the underlying energy landscape, the accuracy of such generative model may still be limited. In this work, we explore the few-shot setting of such pre-trained generative sampler which incorporates MD simulations in a tractable manner. Specifically, given a target protein of interest, we first acquire some seeding conformations from the pre-trained sampler followed by a number of physical simulations in parallel starting from these seeding samples. Then we fine-tuned the generative model using the simulation trajectories above to become a target-specific sampler. Experimental results demonstrated the superior performance of such few-shot conformation sampler at a tractable computational cost.

==> tables/runtime.tex <==
\begin{table}[!ht]
    \centering
    % \footnotesize
    % \small
    \caption{The runtime profiling of different samplers used in this study (unit: wall clock hours).  }
    \label{tb:runtime}
    \begin{tabular}{c|ccc}
    \toprule[1pt]
    Name & MD (100ns) & NE (100 x 1ns) & Diffusion Sampling \\
    \midrule
    BBA & 3.62 & 2.62 & 0.05 \\
    Villin & 2.93 & 2.61 & 0.05 \\
    Trp-cage & 2.73 & 2.12 & 0.09 \\
    BBL & 3.24 & 2.58 & 0.07 \\
    A3D & 4.15 & 3.03 & 0.17 \\
    Chignolin & 2.86 & 1.97 & 0.04 \\
    WW domain & 3.98 & 2.81 & 0.07 \\
    Lambda & 4.34 & 3.06 & 0.20 \\
    NTL9 & 3.63 & 2.53 & 0.08 \\
    Protein G & 3.48 & 2.76 & 0.11 \\
    Protein B & 3.51 & 2.87 & 0.10 \\
    Homeodomain & 6.10 & 4.16 & 0.11 \\
       
        \bottomrule[1pt]
    \end{tabular}
\end{table}
